Commonsense Reasoning for Legged Robot Adaptation with Vision-Language Models

Legged robots are physically capable of navigating a diverse variety of environments and overcoming a wide range of obstructions. For example, in a search and rescue mission, a legged robot could climb over debris, crawl through gaps, and navigate out of dead ends. However, the robot's controller needs to respond intelligently to such varied obstacles, and this requires handling unexpected and unusual scenarios successfully. This presents an open challenge to current learning methods, which often struggle with generalization to the long tail of unexpected situations without heavy human supervision. To address this issue, we investigate how to leverage the broad knowledge about the structure of the world and commonsense reasoning capabilities of vision-language models (VLMs) to aid legged robots in handling difficult, ambiguous situations. We propose a system, VLM-Predictive Control (VLM-PC), combining two key components that we find to be crucial for eliciting on-the-fly, adaptive behavior selection with VLMs: (1) in-context adaptation over previous robot interactions and (2) planning multiple skills into the future and replanning. We evaluate VLM-PC on several challenging real-world obstacle courses, involving dead ends and climbing and crawling, on a Go1 quadruped robot. Our experiments show that by reasoning over the history of interactions and future plans, VLMs enable the robot to autonomously perceive, navigate, and act in a wide range of complex scenarios that would otherwise require environment-specific engineering or human guidance.

==> scratch.tex <==

Legged robots are physically capable of navigating a diverse variety of environments and overcoming a wide range of obstructions. For example, in a search and rescue mission, a legged robot could climb over debris, crawl through gaps, and navigate out of dead ends. However, the robot's controller needs to respond intelligently to such varied obstacles, and this requires handling unexpected and unusual scenarios successfully. This presents an open challenge to current learning methods, which often struggle with generalization to the long tail of unexpected situations without heavy human supervision. To address this issue, we investigate how to leverage the broad knowledge about the structure of the world and commonsense reasoning capabilities of vision-language models (VLMs) to aid legged robots in handling difficult, ambiguous situations. We propose a system, VLM-Predictive Control (VLM-PC), combining two key components that we find to be crucial for eliciting on-the-fly, adaptive behavior selection with VLMs: (1) in-context adaptation over previous robot interactions and (2) planning multiple skills into the future and replanning. We evaluate VLM-PC on several challenging real-world obstacle courses, involving dead ends and climbing and crawling, on a Go1 quadruped robot. Our experiments show that by reasoning over the history of interactions and future plans, VLMs enable the robot to autonomously perceive, navigate, and act in a wide range of complex scenarios that would otherwise require environment-specific engineering or human guidance. Videos of our results can be found on our website: \url{https://vlm-adapt.vercel.app/}.








    

        
    





In this work, we investigate ways to leverage the history of states and behaviors to enable better decision-making with a VLM as the robot learns more about its environment. Our method, Contextual Adaptation from Robotic Errors (CARE), uses a pre-trained VLM to provide behavior commands dynamically. Through in-context learning, by analyzing past behaviors and outcomes, the robot can adjust its strategies to improve performance in future encounters with similar obstacles. This method involves continuous learning from previous experiences, where the robot updates its understanding of what actions are most effective in specific contexts. With CARE, the robot becomes progressively more adept at handling diverse and unpredictable scenarios.





\paragraph{General Setup for All Methods.}
Each method follows a general framework that interacts with a VLM (specifically GPT-4o) to direct the robot's actions based on visual input and historical context. The robot's task is to navigate towards specific objectives (e.g., locating a "red ball") or making forward progress when objectives are not specified. The VLM outputs motor commands after reasoning about the current context and historical data. If progress is not achieved, the model is prompted to reconsider its strategy and choose an alternative behavior.
For each method the VLM is prompted to conclude with 3 words: a yes/no indicating whether progress was made on the prior state with the previous command, the next action command, and a magnitude (Small, Medium, Large) that indicates the extent of the action to take. 















